Soft Merging: A Flexible and Robust Soft Model Merging Approach for Enhanced Neural Network Performance

Stochastic Gradient Descent (SGD), a widely used optimization algorithm in deep learning, is often limited to converging to local optima due to the non-convex nature of the problem. Leveraging these local optima to improve model performance remains a challenging task. Given the inherent complexity of neural networks, the simple arithmetic averaging of the obtained local optima models in undesirable results. This paper proposes a {\em soft merging} method that facilitates rapid merging of multiple models, simplifies the merging of specific parts of neural networks, and enhances robustness against malicious models with extreme values. This is achieved by learning gate parameters through a surrogate of the $l_0$ norm using hard concrete distribution without modifying the model weights of the given local optima models. This merging process not only enhances the model performance by converging to a better local optimum, but also minimizes computational costs, offering an efficient and explicit learning process integrated with stochastic gradient descent. Thorough experiments underscore the effectiveness and superior performance of the merged neural networks.

==> sections/background.tex <==
\section{Related definitions} \label{definitions}
\subsection{Model combination or aggregation} \label{section3:comb}
While model combination or aggregation follows a different track from model merging, it is essential to explain them as related topics to avoid confusion. In this paper, a model refers to the realization of a specific neural network architecture. The model combination is closely related to ensemble learning \cite{opitz1999popular} and auto machine learning \cite{he2021automl}. The model combination involves creating a new architecture from several existing neural network architectures. This contrasts with model merging, where only one architecture is used, and the weights from existing models are mathematically combined. On the other hand, model aggregation refers to utilizing several existing models, which could be in the same architecture or not. It employs mathematical methods to manipulate the results of the models, aiming to achieve improved performance, as demonstrated in the work by  \cite{papernot2016semi}. Model combination or aggregation operates at the architecture level, creating new architectures.

\subsection{Hard merging} \label{section3:hard}
Consider two neural networks, $\mathcal{M}_1$ and $\mathcal{M}_2$, sharing the same architecture. Within each network, the $l$-th layer comprises neurons denoted as $\bbN^{(l)}_1$ and $\bbN^{(l)}_2$, which could represent various components like kernels in Convolutional Neural Networks (CNN) or heads in attention modules.
If $\bbN^{(l)}_1$ has $I$ neurons as $\{\bbn^{(l)}_1[i]\}_i, i=1,...,I$, and $\bbN^{(l)}_2$ has $I$ neurons, denoted as $\{\bbn^{(l)}_2[i']\}_{i'}, i'=1,...,I$, some of these neurons such as $\bbn^{(l)}_1[i]$ and $\bbn^{(l)}_2[i']$ could be matching neurons. Matching neurons are those that approximate each other but may have different spatial locations within the same layer of the architecture \cite{samuel2022git}. The hard merging is generating a new neuron as $\bbn^{(l)}[i]:=f(\bbn^{(l)}_1[i], \bbn^{(l)}_2[i'])$, where $f(\cdot)$ could be any linear or nonlinear function, and it changes the neuron values. 

\subsection{Soft merging} \label{section3:soft}
In contrast to hard merging, soft merging does not alter the values of individual neurons. Building upon the previous example in Section \ref{section3:hard}, soft merging involves selecting $I$ neurons from the combined set of $2I$ neurons, which includes $\{\{\bbn^{(l)}_1[i]\}_i, \{\bbn^{(l)}_1[j]\}_j\}$. The Naive approach for choosing correct neurons would produce computation complexity as $\mathcal{O}({2I \choose I})$ for each layer. Despite its higher complexity, soft merging offers two significant advantages. Firstly, it is a robust method, meaning that even if one model contains extreme values, soft merging remains unaffected. Secondly, soft merging is flexible in terms of choosing which parts to merge. It allows for selective merging of specific layers with given layers.






==> sections/relatedwork.tex <==
\section{Related Works} \label{relatedwork}
